Preconditioning via Diagonal Scaling

Interior point methods solve small to medium sized problems to high accuracy in a reasonable amount of time. However, for larger problems as well as stochastic problems, one needs to use first-order methods such as stochastic gradient descent (SGD), the alternating direction method of multipliers (ADMM), and conjugate gradient (CG) in order to attain a modest accuracy in a reasonable number of iterations. In this report, we first discuss heuristics for diagonal scaling. Next, we motivate preconditioning by an example, and then we study preconditioning for a specific splitting form in ADMM called graph projection splitting. Finally we examine the performance of our methods by some numerical examples.

==> leftright.tex <==

\section{Left and right preconditioners in ADMM}
Consider the problem 
    \begin{equation}
    \begin{array}{ll}
    \mbox{minimize}  & f(x)+g(z) \\
    \mbox{subject to} & Ax+Bz=c, \\
    \label{prob}
    \end{array}
    \end{equation}
with variables $x\in\reals^n$ and $z\in\reals^m$, where $f:\reals^m\rightarrow\reals \cup
\{+\infty\}$ and $g:\reals^m\rightarrow\reals \cup\{+\infty\}$ are convex, closed, and proper functions.
The augmented Lagrangian for this problem is 
\begin{equation}
L_1(x,z,y)=f(x)+g(z)+y^T(Ax+Bz-c)+(1/2)\|Ax+Bz-c\|_2^2,
\label{augmented}
\end{equation}
and the ADMM steps for this problem are \cite{admm:2010}
\begin{equation}
\begin{array}{lll}
x^{k+1} & = &\argmin_xL_1(x,z^k,y^k)\\
z^{k+1} & = & \argmin_zL_1(x^k,z,y^k)\\
y^{k+1} & = & y^k+\left(Ax^{k+1}+Bz^{k+1}-c\right).
\label{ADMM}
\end{array}
\end{equation}
Notice that in our formulation of ADMM, there is no parameter $\rho$ involved in the equations.
We can rewrite the linear constraint in \eqref{prob} as $DAE\tilde x+DBE\tilde z = Dc$, where
 $\tilde x = E^{-1}x$ and $\tilde z = E^{-1}z$. We call $D$ a \emph{left preconditioner} and 
 $E$ a \emph{right preconditioner}.
 
\subsection{Left preconditioners}
\label{leftprec}
Consider the following problem 
    \begin{equation}
    \begin{array}{ll}
    \mbox{minimize}  & f(x)+g(z) \\
    \mbox{subject to} & DAx+DBz=Dc, \\
    \label{newprob}
    \end{array}
    \end{equation}
which is equivalent to \eqref{prob} when $D$ is a diagonal matrix with positive entries on the 
diagonal. The augmented Lagrangian for this problem will be
\begin{equation}
L_D(x,z,y)=f(x)+g(z)+(Dy)^T(Ax+Bz-c)+(1/2)\|Ax+Bz-c\|_{D^2}^2.
\label{augmentedD}
\end{equation}
Defining $Dy$ as the new dual variable, we see that \eqref{augmentedD} is identical to 
\eqref{augmented} except that a different norm is used to augment the Lagrangian. 
Taking $D=\sqrt \rho \mathbf I$, will give us the well-known formulas for ADMM with 
step size $\rho$ introduced in \cite{admm:2010}. Hence, choosing the best left preconditioner is at 
least as difficult as finding the optimal step size $\rho$ in \cite{admm:2010}. 
A question of our interest here is the following: by expanding the class of matrices $D$
from multiples of identity to diagonal matrices, how much can we accelerate the ADMM?
In section \ref{example} we will present an example to illustrate the advantage from this expansion.


\subsection{Right preconditioners}
Consider the following problem where $\tilde x = E^{-1}x$ and $\tilde z = E^{-1}z$.
    \begin{equation}
    \begin{array}{ll}
    \mbox{minimize}  & f(E\tilde x)+g(E \tilde z) \\
    \mbox{subject to} & AE\tilde x+BE\tilde z= c. \\
    \label{newprob2}
    \end{array}
    \end{equation}
It can be easily seen that this problem is equivalent to \eqref{prob}. It can also be verified that 
the ADMM steps for \eqref{newprob2} are identical to those of \eqref{ADMM}.

Hence, we see that choosing a right preconditioner does not have any effect on the
convergence when we are working in infinite precision. In finite precision, however, the choice 
of right preconditioner is a second-order issue. Thus, we will primarily focus on left preconditioners. 


==> proof.tex <==
\section*{Appendix}
\begin{lemma}
Let $A\in\reals^{n\times n}$ be invertible and define $\psi(A)=\|A^{-1}\|\left(\max_j \|A_j\|_2\right)$,
where $A_j$ is the $j^{\mathrm{th}}$ column of $A$.
Assume that $\hat D$ is chosen such that all columns of $A\hat D$ have equal norms. 
Then we will have
\[
\psi(A\hat D) = \inf_D\psi(AD).
\]
\end{lemma}

\begin{proof}
Without loss of generality assume that $\hat D = \bf I$. Then $\max_j \|(AD)_j\|_2 = 
\|A_1\|_2 \max_i D_{ii}$, and $\|(AD)^{-1}\| \geq  \|A^{-1}\|/\max_i D_{ii}$.
\end{proof}

\begin{lemma}
Let $A\in\reals^{n\times n}$ be invertible and choose $\hat D$ such that all columns of $A \hat D$
have equal norms. Then
\[
\kappa(A\hat D) \leq \sqrt{n} \inf_D\kappa(AD).
\]
\end{lemma}

\begin{proof}
Notice that
\BEAS
\kappa(AD) &=& \|(AD)^{-1}\|\|AD\| \\
& = & \psi(AD)\frac{\|AD\|}{\max_j \|(AD)_j\|_2} \\
& \geq & \psi(AD) \\
& \geq & \psi(A\hat D) \\
& = & \|(A\hat D)^{-1}\|\max_j \|(A\hat D)^{-1}_j\|_2\\
& \geq & \|(A\hat D)^{-1}\|\frac{\|A\hat D\|}{\sqrt n} \\
& = & \frac{\kappa(A\hat D)}{\sqrt n}\\
\EEAS
\end{proof}
Now we are ready to prove theorem \ref{theoremvan}.
\begin{proof}
Since $P\in\symm^n_{++}$, it can be written as $P=AA^T$. It is easy to see that the 
columns of $A\hat D$ have equal norms. So
\BEAS
\kappa(DPD) &=& \kappa(AD)^2 \\
& \geq & \frac{\kappa(A\hat D)^2}{n} \\
& = & \frac{\kappa(\hat D P \hat D)}{n} \\
\EEAS
\end{proof}
